Leveraging Internet Principles to Build a Quantum Network

Designing an operational architecture for the Quantum Internet is challenging in light of both fundamental limits imposed by physics laws and technological constraints. Here, we propose a method to abstract away most of the quantum-specific elements and formulate a best-effort quantum network architecture based on packet switching, akin to that of the classical Internet. This reframing provides an opportunity to exploit the many available and well-understood protocols within the Internet context. As an illustration, we tailor and adapt classical congestion control and active queue management protocols to quantum networks, employing an architecture wherein quantum end and intermediate nodes effectively regulate demand and resource utilization, respectively. Results show that these classical networking tools can be effective in managing quantum memory decoherence and maintaining end-to-end fidelity around a target value.

==> background.tex <==
\section{Quantum Background}\label{background}


\subsection{Elements of Quantum Information}
The first postulate of quantum mechanics states that any physical system has a complex vector space associated with it known as the state space of the system. Unit vectors can describe all possible physical states that the system can take in said space \ref{mike&ike}. The smallest model for such systems is a two-dimensional system called a qubit or a quantum bit which resides in the orthonormal basis spanned by vectors $\ket{0} = [1, 0]^T, \ket{1} = [0, 1]^T$. The so-called "ket" $\ket{.}$ formalism is from a shorthand known as Dirac notation. An arbitrary state in this system can be represented as $\ket{\psi} = a\ket{0} + b\ket{1}$
where $a, b \in \mathbb{C}$ and $|a|^2 +|b|^2 = 1$. 'Superposition' is exactly this: the ability of the system to be in a linear combination of two or more possible states with complex scalar factors. Measurements make the superposition collapse on only one of its components. Physical systems that qubits can model are numerous e.g. polarization of photons, atomic particle spins, photon space-time trajectories, etc. The evolution of closed systems is described by unitary transformations e.g. $\ket{\psi}’ = U\ket{\psi}$ describes the evolution of state $\ket{\psi}$ to $\ket{\psi}’$ under the process $U$.

\subsubsection{Quantum Noise}
Quantum Noise can be described as unwanted transformations that a system can undergo due to interactions with the environment as no quantum system is perfectly isolated.
This probabilistic nature of noise gives rise to what is known as mixed states i.e., a probabilistic ensemble of pure quantum states. One particular mixed state of interest is the maximally mixed state i.e. the mixed state which is formed by having a uniform distribution over all possible states. It is the model for a state that essentially contains no useful information or completely scrambled information.

One of the most widely adopted models for quantum noise is the \emph{depolarizing channel}. This replaces a qubit state with a maximally mixed state with a certain depolarization probability. In other words, it scrambles the information stored in the qubit, resulting in more information loss. It is often used as a worst-case noise model due to its isotropic, disruptive effect. A physical example of such a process is light scattering after hitting atomic particles causing scrambling of the polarization.

\emph{Fidelity} is a well-known metric that quantifies the "amount" of noise a quantum system has undergone by measuring the distance between a reference and the actual quantum state.  

Most models assume three sources of noise on a quantum network: (i) Initial imperfections (no qubit state is created perfectly), (ii) imperfect quantum gates, and (iii) quantum memory decoherence, which progressively degrades the fidelity of qubit states stored in memories. All these noises are often mapped to depolarizing channels.

\subsubsection{Entanglement}
 Quantum entanglement is a phenomenon with no classical counterpart in which one cannot describe the quantum state of a composite system as the separated quantum states of its subsystems. The consequence is that, even if the subsystems are geographically separated, they still share a single quantum state. Focusing on two-qubit states, the most famous example of such a state is the \emph{Bell state} $\ket{\Phi^+} = (\ket{00} +\ket{11})/\sqrt{2}$. Bell states are maximally entangled: measuring one qubit also fully collapses the other to either $\ket{0}$ or $\ket{1}$. One possible interpretation of this phenomenon is that there are interactions possible in nature that correlate the properties of two systems in such a manner that it becomes impossible to describe the two systems separately. There are many examples of physical processes that lead to entanglement. For example, an ion and a photon emitted by excitation of said electron and spontaneous parametric down-conversion.

\subsubsection{Quantum Teleportation}
Quantum teleportation is a protocol through which one can transfer the state of one qubit using a pre-shared Bell pair, local quantum operations, and classical communication. Consider two parties Alice and Bob holding each a half of a Bell pair. Alice also holds a third qubit in an arbitrary state $\ket{\psi}$ she wants to send to Bob. She carries out an operation called \acf{BSM} and sends the measurement outcome (two classical bits) via classical communication to Bob, who uses it for a simple correction. The Bell pair has been consumed in the measurement, but now Bob holds the state $\ket{\psi}$ in the qubit that used to be his half of the Bell pair. Note that only classical information has been transmitted over the network. The primary benefit of quantum teleportation over direct transmission of the qubit state is that the state being teleported is shielded from noise and loss that can occur during physical transmission, a major issue in quantum communication.

Now that we established that we can transmit qubit states on top of pre-shared entanglement, the primary role of the quantum network becomes the continuous generation and distribution of entanglement to enable connectivity through teleportation.

\textbf{Takeaway message:} \textit{Quantum networks will use entanglement as an expendable resource to enable quantum communication.}

\subsection{Entanglement Distribution}

\subsubsection{Link-level Entanglement Generation}

\ac{LLEG} is the elementary process that generates and distributes Bell pairs shared between two parties connected through some physical medium, i.e. fiber or open space. The direct connection here means that qubit states can be physically transmitted between the two parties. Literature has produced several \ac{LLEG} protocols \cite{Munro_2015} that depend on the adopted hardware platform. What is common to all these protocols is that \ac{LLEG} is intrinsically probabilistic: attempts succeed with a probability $p$ that usually depends on the efficiency and brightness of the photon source \gv{Maybe better to say "brightness" of the photon source?} \LB{Fixed}, the efficiency of frequency coupling, medium attenuation, and link length. 

Due to its probabilistic nature, we model \ac{LLEG} as a discrete stochastic process where every sample is an independent, identically distributed geometric random variable $K$ distributed according to $P(K=k) = p(1-p)^{k-1}$, where $k\geq1$ is the number of attempts to success. The inter-generation time $T$ between successful \ac{LLEG} attempts is thus $T=K/f_a$, where $f_a$ is the attempt frequency of the protocol.

\subsubsection{Quantum Repeaters}
Direct communication imposes distance limits for physical links as photons suffer exponential loss through optical fiber. This poses a major challenge in classical networks too. Unlike classical signals, one cannot even amplify quantum signals: copying quantum information is prohibited by the well-known no-cloning theorem of quantum mechanics. As a result, we cannot solely employ \ac{LLEG} to distribute entanglement if the parties are too distant from each other.

Quantum repeaters are a workaround to this problem. Their role is to employ \ac{LLEG} to get short-distance Bell pairs and then stitch these together using entanglement swapping to create a longer-distance Bell pair.
Entanglement Swapping is a specific instance of quantum teleportation where the qubit being teleported is itself one-half of a Bell pair. This overcomes the issues of photonic loss in direct communication allowing for sharing Bell pairs across --in theory-- arbitrarily long distances.

==> dynamic_rendez_vous.tex <==

\section{Connectionless Network Protocol}\label{sec:conn_network_prot}

    We describe here a Network layer protocol to propagate entanglement to the end nodes. The protocol is best-effort and connectionless by design, meaning that quantum nodes do not reserve any resource in advance and treat every request independently. These properties match packet forwarding in the classical Internet, making this one of the foundations on which we build our results.
    
    \subsection{Sequential Swapping}
        Following the example in Fig. \ref{fig:timing_seq}, suppose that an end node $v_0$ wants a Bell pair with another end node $v_3$. From a physical perspective, we adopt a \emph{Sequential entanglement swapping policy} on the repeaters $v_1$ and $v_2$. As shown in Fig. \ref{subfig:seq_a}, this policy has a repeater start \ac{LLEG} on the next link only after it is directly entangled with the source node $v_0$. When \ac{LLEG} succeeds, the repeater carries out entanglement swapping between the communication qubit and the target storage qubit. Finally, it notifies the next node.
        
        From a networking perspective, we see in Fig. \ref{subfig:seq_b} that Sequential swapping is implemented through a classical packet called \emph{entanglement request} which is forwarded hop by hop as \acp{BSM} occur. The entanglement request collects and conveys the classical information required by the destination end node $v_3$ to determine the \ac{e2e} Bell state. The next hop to which the node should forward a request is determined when the request arrives by a Quantum Routing protocol that is out of the scope of this work. We could assume here to use shortest path routing such as the \ac{OSPF} protocol. The entanglement request queues, introduced in Fig. \ref{fig:sys_model}, address the necessity of storing entanglement requests for the time needed until the communication qubit can be used to swap and forward the request.
    
        
        
        \begin{figure*}
            \begin{centering}
                \subfloat[Sequential swapping]{\includegraphics[height=0.4\linewidth]{img/TimingSeqA.pdf} \label{subfig:seq_a}} \hspace{1cm}
                \subfloat[Time Diagram] {\includegraphics[height=0.4\linewidth]{img/TimingSeqB.pdf}\label{subfig:seq_b}}
            \end{centering}
            \centering
            \caption{Example time sequence of the sequential swapping policy. The figures track a) the state of the entangled qubits and b) the classical signals exchanged by nodes during the operations. Red and green lines highlight the heralding of failed and successful \ac{LLEG} respectively. Mail icons represent entanglement request packets. requests are also forwarded to the link controllers so that they can start \ac{LLEG}.}
            \label{fig:timing_seq}
        \end{figure*}

    \subsection{Bidirectional Swapping}
        Suppose that the same end nodes $v_0$ and $v_3$, instead of a single Bell pair, want to share a whole flow of Bell pairs over time --e.g., for a \ac{QKD} application. The end nodes then start generating entanglement requests that, once delivered, will be mapped to the same flow by the Transport layer protocol. Here comes a major departure from classical networking: quantum entanglement distribution is a symmetric process that can be initiated by either of the two end nodes. We assume then that entanglement flows have two request sources instead of a source and a destination, which is the case for classical \ac{TCP} flows. In our model, repeaters forward entanglement requests in both directions along a path connecting $v_0$ and $v_3$.

    %\subsection{Dynamic Rendez-vous Protocol}
        %Now that we introduced bidirectional, Sequential swapping, it follows that requests that belong to the same flow and travel in opposite directions can meet at any intermediate repeater on the path. Instead of treating them as independent requests, the repeater can free up resources earlier by carrying out a \ac{BSM} on the two storage qubits associated with the two requests. The end nodes share now a Bell pair, and the repeater sends an acknowledgment message to both end nodes so that they know that the requests have been fulfilled (and the resulting \ac{e2e} Bell state). The dynamic rendez-vous protocol adds some complexity at the core of the quantum network, but it can substantially improve the performances, as we will show later in this work. We show an example sequence of the dynamic rendez-vous protocol in Fig. \ref{fig:timing_rend}, where the rendez-vous happens at $v_2$. In the example. both $v_0$ and $v_3$ generate a request at roughly the same time (step I). The two requests eventually meet at $v_2$, which carries out the rendez-vous (step VI).

        %\begin{figure*}
            %\begin{centering}
                %\subfloat[Dynamic Rendez-vous]{\includegraphics[height=0.4\linewidth]{img/TimingRendezA.pdf} \label{subfig:rend_a}} \hspace{1cm}
                %\subfloat[Time Diagram] {\includegraphics[height=0.4\linewidth]{img/TimingRendezB.pdf}\label{subfig:rend_b}}
            %\end{centering}
            %\centering
            %\caption{Example time sequence of the bidirectional, sequential swapping policy with dynamic rendez-vous. The figures track a) the state of the entangled qubits and b) the classical signals exchanged by nodes during the operations. Red and green lines highlight the heralding of failed and successful \ac{LLEG} respectively. Mail icons represent entanglement request packets.}
            %\label{fig:timing_rend}
        %\end{figure*}
    

==> eval.tex <==
\section{Evaluation}

In this section, we evaluate the effect of congestion control and AQM on the queue size, throughout, and the dropping rate of requests for entanglement generation in a repeater chain. 

\subsection{Experiment setup}

We use a simple repeater chain with only three repeaters in the experiments. The length of each link is $50$ km. Due to photon loss in the fiber,  link-level entanglement generation is probabilistic, and the success probability is given by
\begin{align}
    \label{eq:link-level-prob}
    p_i = p_\text{link} e^{-\alpha L_i},  
\end{align}
where $\alpha$ is the fiber attenuation rate, $L_i$ is the length of the fiber for the $i$-th link, and $0\leq p_\text{link}\leq 1$ accounts for fiber coupling efficiency, detector efficiency, etc. Here, we set $\alpha= 0.046~[\text{km}^{-1}]$ corresponding to $0.2$~dB/km signal attenuation in fiber and $p_\text{link}=1$ for simplicity.

We assume each repeater has the capacity $c$ and that all interfaces can use the memories. There are $\cF$ flows in the repeater chain. 


\subsection{Stability with AQM}

Figure \ref{fig:aqm} shows the queue delay, end-to-end fidelity, and drop rate of the repeater chain in the presence and absence of AQM and congestion control in the network. Figure \ref{fig:aqm}.a shows how long it takes the network to achieve a stable state under different setups. 


\begin{figure*}
\centering
\includegraphics[scale=0.71]{img/drop_rate_e2e_f_delay.pdf}
% \vspace{-0.1in}
\caption{(Cartoon graph)Drop rate, request service delay, and e2e fidelity in the presence and absent fo AQM.}
\label{fig:aqm}
\end{figure*}



\subsection{Throughput}




==> protocol.tex <==

\subsection{Protocol}

Here we explain the protocol by explaining the packet types and the triggered events upon arriving each of them at nodes in the system.

\textbf{Packet types:} There are five different types of packets in our connectionless entanglement distribution network:

\begin{enumerate}
    \item  \textbf{Request packet} that includes the request ID, flow ID, and the source and destination node ID and the LLE ID. We assume when the source node receives a request, the packet has a default ID for the LLE ID and it will generate the request ID for it. The source node is the only node that creates a unique ID for the request. 
    
    \item \textbf{Swap packet} that contains the request and flow ID and the source node ID for that request.
    
    \item \textbf{Canceling packet} that indicates a buffer overflow and contains the request and flow ID and the EPR ID.
    
    \item \textbf{EPR lock packet} that is used when a node wants to perform a swap operation on a pair of qubits. We call this packet a \textit{lock packet} as it locks an EPR pair. We need the lock packets to prevent two nodes from performing swap operations on the same LLE pairs for the same or two different flows in opposite directions. Nodes use this packet to ask the adjacent node to lock a specific EPR pair and prevent inconsistency. These packets include the EPR and flow ID. If a node has already sent a lock message for the specific EPR pair that is mentioned in the received lock packet, it will reply "no" (in the acknowledgment type packet) to the sender. 
    
    \item \textbf{Acknowledgment packet} that would be sent in response to a lock packet and include "yes" or "no".  
 
\end{enumerate}

\subsubsection{Events}
There could be multiple events in the system that we explain in the following section. 

\textbf{Upon receiving a request packet:} When a node receives a request packet, it will first check if it has enough memory in its queue. If it does not have enough memory for the request, it will drop the packet and trigger the congestion control function. The congestion control function may or may not react to each call. If the queue is full and it is a source node, it does not need to do anything else. For the other nodes when the queue is full, they will send a canceling packet containing the request and the source node ID to the upper stream node. If the node has enough buffer in its queue it will append the request to the queue. Note that if the node is a source node, it will generate a unique ID for the request and then append it to the queue.  


\textbf{Upon receiving a lock packet:} When a node receives a lock packet for an EPR pair from its adjacent neighbor, the node will first check if it has already sent a lock packet for that EPR pair or not and it will reply with a "no" flag in the acknowledgment message if it has. If it has marked the EPR pair as available, it will again send a "no" message to the sender. Otherwise, it will mark the EPR pair indicated by the packet as unavailable and reply to it with an acknowledgment packet. 

\textbf{Upon receiving an acknowledgment packet:} The node will first flag the LLE pair indicated by the packet as unavailable and then will perform a swap on the qubit of this LLE and the qubit of the EPR pair attached to the request and send a request message to the downstream node. It will send a swap message to the upper stream node also. The swap message will be forwarded to the source node of the request. 

\textbf{Upon receiving a canceling packet:}  The node will drop the request (indicated by the request packet) from the queue and send a canceling packet to the upper stream node if the node is not the source node and trigger the congestion control function. Otherwise, it will do nothing. 

\textbf{Upon receiving a swap packet:} If the node is not the source node of the request, it will back forward the swap packet to the upper stream node. Note that this works for a repeater chain. If it is a general network, the node may ignore the swap packet for the requests that it has not done any swap for it. If it is a source node, if it has received a swap from all the intermediate nodes, that means the end-to-end entanglement has been generated and it can perform an operation such as teleportation on the qubit.

\textbf{Upon receiving congestion control signal:} The congestion control signal at a node will be triggered if a node drops a request or receives a canceling message or if it receives the signal from the timer. We assume there is a timer that triggers the congestion control controller every $T$ seconds. At this point, the node will check the average size of the request queue and LLE pairs queue and update the pump power according to a set of rules, and update the sending rate if it is the source node.

Each node in a loop will check the request queue and if there is any queue, it will pick the oldest one and check if there is any free LLE in its queue. If there is any, it will choose the youngest one and send a lock message including the ID of the chosen EPR pair to the downstream node. Otherwise, it will wait until there is one LLE pair generated. Note that this packet includes enough information that help the node know the swap operation should be performed on which pair of qubits.

==> rel.tex <==

\section{Related work}

Could the system of the previous papers be unstable?  They may keep switching between routes in different periods. The previous papers do not talk about stability. It is possible that the network they have used is such that their protocol and algorithm behave nicely. 

==> unprocessed.tex <==


\subsubsection{Computing e2e fidelity}

Assume the dephasing noise at each switch is $F(t) = c_1+c_2e^{-t/T_c}$ where $c_1+c_2= 1$ and $t$ is memory life time. Note $i=0$ is the end node and $i=1,...,n$ corresponds to memories at the end of link $i$. $T_c$ is the coherence time of the memory.

$T_i$ is the time for request to pass through link $i$, $T_i\sim Exp(\mu_i-\lambda)$ and $T$ is total time = $\sum_{i=1}^{n}T_i$. $T_i^{*}(s) = E(e^{-sT_i}) = \frac{\mu_i-\lambda}{\mu_i-\lambda+s}, T^*(s) = E(e^{-sT})=\prod_{i=1}^nT^*_i(s)= \prod_{i=1}^n\frac{\mu_i-\lambda}{\mu_i-\lambda+s}$ 


Let $F$ be the fidelity of the final EPR pair with an average $\overline{F}$ then we can have the following cases:
\begin{enumerate}
    \item Assume zero classical communication delay and that qubit of EPR pair at end node remains in memory, and that a request at link $i$ waits for next LLE, then $\overline{F}=T^*(2/T_c) = \prod^n_{i=1}\frac{\mu_i-\lambda}{\mu_i-\lambda+1/T_c}$

    \item If end node qubit is consumed immediately, then $\overline{F} = T^*(1/T_c)$
    \item Suppose classical communication suffers latency $L_i$ over link $i$, and end node qubit remains in memory and $L=\sum_{i=1}^{n}L_i$, then $\overline{F}= T^*(2/T_c)e^{-2L/T_c}*e^{-2L/T_c}$ where the first $e^{-2L/T_c}$ is for correction and the second $e^{-2L/T_c}$ is for the heralding delay.
    \item Assuming two cases of (2) and (3) we have  $\overline{F} = T^*(1/T_c)e^{-2L/{T_c}}$
\end{enumerate}




\subsection{General network}

We assume we have fixed paths $P\subset E$ (that need to be contiguous links) and request accompany distribution at each switch has product form (infinite memory), assume coherence time $T_c$ for all memories and let $F_f$ denote fidelity for flow $f$ then $\overline{F}_f = \prod_{i\in f}\frac{\mu_i-\sum_{g\ni i}\lambda_i}{\mu_i-\sum_{g\ni i}\lambda_i+s} \forall f\in \cF$

The last equation needs to be checked.
\subsubsection{Remarks:}


\begin{enumerate}
    \item If flows are always in the same direction across a link, it can allow for storage of a finite number of LLEs provided served oldest first.
    \item Seems plausible that we can numerically compute $F$ when requests are served locally youngest first
\item Huge literate developing approximations, limits, bounds for a general network that violate product form assumptions.
\begin{enumerate}
    \item General arrival processes
    \item Finite capacity memoirs
\end{enumerate}
\item GHZ states $\rightarrow$ Task queuing systems $\rightarrow$ Many approximations ...
\end{enumerate}

\subsubsection{A scheduling result}

For a linear network with single flow, $\overline{F}$ is maximized by a policy that always serves globally youngest request (not to be confused with locally youngest requests)\cite{towsley1991comparisons}

Remark: This may hold more generally in a multi-flow system where the result holds on a per-flow basis.
